Atrial Fibrillation Detection Using RR-Intervals for Application in Photoplethysmographs

Atrial Fibrillation is a common form of irregular heart rhythm that can be very dangerous. Our primary goal is to analyze Atrial Fibrillation data within ECGs to develop a model based only on RR-Intervals, or the length between heart-beats, to create a real time classification model for Atrial Fibrillation to be implemented in common heart-rate monitors on the market today. Physionet's MIT-BIH Atrial Fibrillation Database \cite{goldberger2000physiobank} and 2017 Challenge Database \cite{clifford2017af} were used to identify patterns of Atrial Fibrillation and test classification models on. These two datasets are very different. The MIT-BIH database contains long samples taken with a medical grade device, which is not useful for simulating a consumer device, but is useful for Atrial Fibrillation pattern detection. The 2017 Challenge database includes short ($<60sec$) samples taken with a portable device and reveals many of the challenges of Atrial Fibrillation classification in a real-time device. We developed multiple SVM models with three sets of extracted features as predictor variables which gave us moderately high accuracies with low computational intensity. With robust filtering techniques already applied in many Photoplethysmograph-based consumer heart-rate monitors, this method can be used to develop a reliable real time model for Atrial Fibrillation detection in consumer-grade heart-rate monitors.

==> links.tex <==
\section*{Relevant Links}
\textit{
The cfg files for each of the trials and their corresponding weights files can be found at \href{https://github.com/reu2018DL/YOLO-LITE}{https://github.com/reu2018DL/YOLO-LITE}. 
The live demo can be found at \href{https://reu2018dl.github.io/}{https://reu2018dl.github.io/}
}

==> unsure_toinclude.tex <==
\subsection{Markov Chain Diagrams}

Because the transition matrix plots did not do any predictions and mostly just identified patterns we chose to look at Markov Chain Diagrams to clearly identify proportions and predictions as a whole for AFib and non-AFib readings. Another reason we looked at Markov Chain Diagrams is that it allowed us to identify the differences in the AFib and non-AFib readings of the same subject in a clear manor. 

To create the Markov Chain Diagrams our first step was to convert our previously used transition proportion matrices into a stochastic left matrix, or a matrix where each column adds to one instead of the entire matrix. This was done so we could determine $P(C_{x_2}|C_{x_1})$ where $x = (1, 2, 3)$; $C_x = (N, S, L)$. Using these new matrices we created an average stochastic matrix for each Subject which was then used to create the Markov Chain Diagrams. To develop this in a way that could be efficiently modelled we used Equation \ref{rmean} to create a running average of the matrix. The diagrams below give the average at the end of each Subjects' ECG readings. 

\begin{figure}[H]
    \centering
    \includegraphics[width = .45\textwidth, keepaspectratio]{photos/tdiagram04048.jpeg}
    \caption{Markov Chain Diagram of Final Running Average of Left Stochastic Matrix of Subject 04048}
    \label{mdia04048}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .45\textwidth, keepaspectratio]{photos/tdiagram07879.jpeg}
    \caption{Markov Chain Diagram of Final Running Average of Left Stochastic Matrix of Subject 07879}
    \label{mdia07879}
\end{figure}
\vspace{.3cm}

Above, Figures \ref{mdia04048} and \ref{mdia07879} show the diagrams of the left stochastic matrices of the previously identified subjects. We can observe a lower $P(N|N)$ in Figure \ref{mdia07879}, which is expected given the distributions we saw earlier. $P(S,L|N)$ is also higher in Figure \ref{mdia07879}. Otherwise, there is not a great difference between the two. Because of the similarities between the two Figures we decided to separate Figure \ref{mdia07879} into AFib and non-AFib left stochastic matrices

\begin{figure}[H]
    \centering
    \includegraphics[width = .45\textwidth, keepaspectratio]{photos/avgtAFib07879.jpeg}
    \caption{Markov Chain Diagram of Final Running Average of Left Stochastic Matrix of AFib Samples in Subject 07879}
    \label{AFib07879}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .45\textwidth, keepaspectratio]{photos/avgtnon07879.jpeg}
    \caption{Markov Chain Diagram of Final Running Average of Left Stochastic Matrix of non-AFib Samples in Subject 07879}
    \label{non07879}
\end{figure}
\vspace{.3cm}

For the separated AFib and non-AFib Markov Chain Diagrams, above, we used the same process of doing the running average specified in Equation \ref{moddyrmean}. The non-AFib Diagram in Figure \ref{non07879} has $P(N|L)=0$ and $P(N|S)=0$, and $P(N|N) = 0.978$, while the AFib Diagram as $P(N|N)=0.718$. This drop in $P(N|N)$ is what we have seen in every other Figure during AFib intervals and may be the best way to determine a dangerous level of AFib. This is because by using the running mean on a Markov Chain Diagram we would not have to store a large amount of data to understand the patterns of the heart rate and may be able to identify a threshold for 'dangerous' levels of AFib.

